Max-Min Rate Fairness Optimization for Multi-User Pinching-Antenna NOMA Systems

Pinching-antenna systems (PASs) can overcome signal blockage by repositioning dielectric radiating elements, called pinching antennas (PAs), along meter-scale waveguides to create line-of-sight links. Since each waveguide is driven by a single radio-frequency (RF) chain, non-orthogonal multiple access (NOMA) is well suited for PAS-based multi-user communications. This paper studies a PAS-enabled multi-user downlink NOMA system with multiple waveguides, each equipped with multiple PAs. The PA positions and base-station transmit precoding are jointly optimized to maximize the minimum user rate. The resulting problem is highly non-smooth and non-convex because of the rapidly oscillating coherent sums caused by inter-PA interference. To tackle this challenge, we propose a two-stage structured optimization framework. In the first stage, coarse PA-position and power-allocation optimization is performed using an interior-point algorithm while neglecting the PA channel phases, which gives solutions near the true optima. In the second stage, PA positions and transmit precoding are fine-tuned while accounting for the PA channel phase shifts. This stage first applies phase zeroing, where each PA is locally repositioned to align the corresponding channel phase toward zero and promote constructive coherent combining. It then uses an alternating procedure that iteratively performs forward-backward PA position refinement and successive-convex-approximation-based complex transmit precoding optimization until convergence, thereby reducing residual phase mismatch. Simulation results show that the proposed framework significantly outperforms heuristic optimization benchmarks with much lower computational time. They also demonstrate large gains over a comparable multiple-input multiple-output downlink NOMA system and reveal the impact of the number of PAs, users, and transmit power on system performance.

==> sys_model.tikz.tex <==

\begin{circuitikz}
\tikzstyle{every node}=[font=\Huge]
\draw [ fill={rgb,255:red,204; green,204; blue,204} , line width=1pt , rounded corners = 0.5] (-2,3) -- (-2.75,3.75) -- (-2.75,0.75) -- (-2,0) -- cycle;
\draw [ fill={rgb,255:red,204; green,204; blue,204} , line width=1pt , rounded corners = 0.5] (-2,3) rectangle (0.25,0);
\draw [ fill={rgb,255:red,204; green,204; blue,204} , line width=1pt, rounded corners = 0.5] (-0.5,3.75) -- (-2.75,3.75) -- (-2,3) -- (0.25,3) -- cycle;
\node [font=\Huge] at (-0.25,2.625) {...};
\draw [line width=1pt, short] (-2,0.75) -- (0.25,0.75);
\draw [line width=1pt, short] (-2,1.5) -- (0.25,1.5);
\draw [line width=1pt, short] (-2,2.25) -- (0.25,2.25);
\draw [line width=1pt, short] (-1.75,2.625) -- (-1,2.625);
\draw [line width=1pt, short] (-1.75,1.875) -- (-1,1.875);
\draw [line width=1pt, short] (-1.75,1.125) -- (-1,1.125);
\draw [line width=1pt, short] (-1.75,0.375) -- (-1,0.375);
\draw  (3,2.75) circle (0cm);
\draw  (4,-2) circle (0cm);
\draw  (4.25,-2.5) circle (0cm);
\draw  (4,-2.5) circle (0cm);
\draw  (4,-2.5) circle (0cm);
\node [font=\Huge] at (-0.25,1.875) {...};
\node [font=\Huge] at (-0.25,1.125) {...};
\node [font=\Huge] at (-0.25,0.375) {...};
\draw [line width=1pt, short] (-1.5,3.75) .. controls (-1.25,6.75) and (-2.75,7.25) .. (3.2,7.25);
\draw [line width=1pt, short] (6.25,3.25) -- (1.25,-3.25);
\draw [line width=1pt, short] (4,8.25) -- (2,5.75);
\draw [line width=1pt, short] (1.25,-3.25) -- (13.5,-3.25);
\draw [line width=1pt, short] (6.25,3.25) -- (18.5,3.25);
\draw [line width=1pt, short] (18.5,3.25) -- (13.5,-3.25);
\draw [line width=1pt, ->, >=Stealth, dashed] (3.75,0) -- (17,0);
\draw [line width=1pt, <->, >=Stealth] (1.25,-3.75) -- (13.5,-3.75);
\draw [line width=1pt, <->, >=Stealth] (0.5,-3.25) -- (5.75,3.5);
\draw [line width=1pt, ->, >=Stealth, dashed] (6.25,3.25) -- (7,4.25);
\draw [line width=1pt, short] (4,8.25) -- (4.75,8.25);
\draw [line width=1pt, short] (2,5.75) -- (2.75,5.75);
\draw [ fill={rgb,255:red,61; green,145; blue,255} , line width=1pt , rounded corners = 3.0] (4.75,8.45) rectangle (6.25,8.05);
\draw [line width=1pt, short] (6.25,8.25) -- (7,8.25);
\draw [ fill={rgb,255:red,198; green,221; blue,251} , line width=1pt , rounded corners = 3.0] (7,8.45) rectangle (19.25,8.05);
\draw [ fill={rgb,255:red,89; green,139; blue,245} , line width=1pt , rounded corners = 3.0] (2.75,5.95) rectangle (4.25,5.55);
\draw [line width=1pt, short] (4.25,5.75) -- (5,5.75);
\draw [ fill={rgb,255:red,194; green,223; blue,255} , line width=1pt , rounded corners = 3.0] (5,5.95) rectangle (17.25,5.55);
\draw [line width=1pt, short] (3.4,7.5) -- (4.25,7.5);
\draw [ fill={rgb,255:red,77; green,142; blue,250} , line width=1pt , rounded corners = 3.0] (4.25,7.7) rectangle (5.75,7.3);
\draw [line width=1pt, short] (5.75,7.5) -- (6.5,7.5);
\draw [ fill={rgb,255:red,196; green,222; blue,253} , line width=1pt , rounded corners = 3.0] (6.5,7.7) rectangle (18.75,7.3);
\node [font=\Huge, rotate around={50:(0,0)}] at (11.5,6.625) {...};
\node [font=\Huge] at (-1,-0.75) {Base};
\node [font=\Huge] at (-1,-1.5) {Station};
\node [font=\Huge] at (7.25,4.75) {$y$};
\node [font=\Huge] at (17.5,0) {$x$};
\node [font=\Huge] at (7.25,-4.5) {$D_1$};
\node [font=\Huge] at (2.5,0.5) {$D_2$};
\node [font=\Huge] at (21.75,8.35) {Waveguide 1};
\node [font=\Huge] at (21.25,7.4) {Waveguide 2};
\node [font=\Huge] at (19.875,5.75) {Waveguide $M$};
\node [font=\Huge] at (5.5,9.1) {RF Chains};
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (8.8,5.75) -- (9.125,5.3) -- (9.45,5.75) -- (9.125,6.2) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (15.8,5.75) -- (16.125,5.3) -- (16.45,5.75) -- (16.125,6.2) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (14.55,5.75) -- (14.875,5.3) -- (15.2,5.75) -- (14.875,6.2) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (17.3,7.5) -- (17.625,7.05) -- (17.95,7.5) -- (17.625,7.95) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (9.55,8.25) -- (9.875,7.8) -- (10.2,8.25) -- (9.875,8.7) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (13.55,8.25) -- (13.875,7.8) -- (14.2,8.25) -- (13.875,8.7) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (16.3,8.25) -- (16.625,7.8) -- (16.95,8.25) -- (16.625,8.7) -- cycle;
\draw [ fill={rgb,255:red,0; green,0; blue,0} ] (8.05,7.5) -- (8.375,7.05) -- (8.7,7.5) -- (8.375,7.95) -- cycle;
\node [font=\Huge, rotate around={-360:(0,0)}] at (4.55,-0.55) {$(0,0)$};
\node at (3.75,0) [circ] {};
\draw [ rotate around={-128:(-0.25, -6.75)}] (-0.25,-6.75) rectangle (-0.25,-6.75);

\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (6.75,2.75) rectangle (8,1);
\draw [ fill={rgb,255:red,255; green,255; blue,254} , line width=1pt , rounded corners = 4.0] (7,2.5) rectangle (7.75,1.25);
\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (6.75,3) rectangle (7,2.25);
\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (11.75,-0.5) rectangle (13,-2.25);
\draw [ fill={rgb,255:red,255; green,255; blue,254} , line width=1pt , rounded corners = 4.0] (12,-0.75) rectangle (12.75,-2);
\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (11.75,-0.25) rectangle (12,-1);
\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (8,-0.5) rectangle (9.25,-2.25);
\draw [ fill={rgb,255:red,255; green,255; blue,254} , line width=1pt , rounded corners = 4.0] (8.25,-0.75) rectangle (9,-2);
\draw [ fill={rgb,255:red,0; green,0; blue,0} , line width=1pt , rounded corners = 4.0] (8,-0.25) rectangle (8.25,-1);
\node [font=\Huge] at (7.375,0.5) {UE 1};
\node [font=\Huge] at (8.625,-2.75) {UE 2};
\node [font=\Huge] at (10.5,-1.25) {...};
\node [font=\Huge] at (12.375,-2.75) {UE $K$};
\draw [line width=1pt, <->, >=Stealth] (12,5.25) -- (12,0.25);
\node [font=\Huge] at (12.5,2.5) {$d$};
\end{circuitikz}
